Harnessing the Power of Many: Extensible Toolkit for Scalable Ensemble Applications

Many scientific problems require multiple distinct computational tasks to be executed in order to achieve a desired solution. We introduce the Ensemble Toolkit (EnTK) to address the challenges of scale, diversity and reliability they pose. We describe the design and implementation of EnTK, characterize its performance and integrate it with two distinct exemplar use cases: seismic inversion and adaptive analog ensembles. We perform nine experiments, characterizing EnTK overheads, strong and weak scalability, and the performance of two use case implementations, at scale and on production infrastructures. We show how EnTK meets the following general requirements: (i) implementing dedicated abstractions to support the description and execution of ensemble applications; (ii) support for execution on heterogeneous computing infrastructures; (iii) efficient scalability up to O(10^4) tasks; and (iv) fault tolerance. We discuss novel computational capabilities that EnTK enables and the scientific advantages arising thereof. We propose EnTK as an important addition to the suite of tools in support of production scientific computing.

==> acknowledgements.tex <==
\footnotesize{Acknowledgments: This work is supported by NSF ICER 1639694,
DOE ASCR DE-SC0016280 and an INCITE award to J.T. This research used
resources of the Oak Ridge Leadership Computing Facility at the Oak Ridge
National Laboratory, which is supported by the Office of Science of the
U.S.Department of Energy under Contract No. DE- AC05-00OR22725.}


==> entk_design-2.tex <==
The design and implementation of EnTK are iterative and driven by use cases.
Use cases span several scientific domains, including Biomolecular
Sciences~\cite {entk-md}, Physics~\cite{entk-physics}, and Earth
Sciences~\cite{entk-heart- science}\mtnote{Please add references and
edit/extend this list as appropriate}. Users and developers collaborate to
describe use cases and elicit requirements in a continuous feedback loop with
rapid prototyping. EnTK is loosely specified in UML and its prototypes are
validated against the current set of requirements and characterized by their
performance. Both Jenkins and Travis are used for continuous integration and
automated testing of every commit. Documentation and code are managed and made
available via a public GitHub repository~\cite{entk-repo}.

\subsection{Requirements}\label{ssec:requirements}

EnTK supports Ensemble-based applications (EBAs), where an ensemble is defined
as a set of tasks. Ensembles may vary in the number of tasks, types of task,
tasks' executable (or executing kernel), and tasks' resource requirements.
EBAs may vary in the number of ensembles or the runtime dependencies among
ensembles. The space of EBAs is vast, and thus there is a need for
simple and uniform abstractions while avoiding single- point solutions. We
elicited requirements of EBA for computing infrastructures (CIs), scale,
fault-tolerance, and usability.

EBAs serve diverse science domains and require CIs ranging from
clusters and grids to clouds. Efficient execution of EBAs on different CIs
poses several technical challenges, neither of which are of interest to
domain scientists. This suggests three requirements for EnTK\@: (1) enabling
the execution of EBAs on heterogeneous CIs; (2) abstract the complexity of
execution and resource management from the user; and (3) keeping the
performance of the framework independent on to the type of CI on which EBAs'
tasks are executed.

Currently, the use cases motivating EnTK require a maximum of \(O(10^4)\)
tasks but EnTK is designed to support up to \(O(10^6)\) tasks due to the rate
at which this requirement has been increasing, especially in biomolecular
simulations where a greater number of tasks is associated with greater sampling or
more precise free energy calculations. Most of the limitations to the scale of the
supported EBAs derive from the runtime used to execute the EBAs' tasks on the
CIs. As such, one of the requirements of EnTK is to be runtime-independent,
enabling the use of different middleware, depending on the requirements of
specific EBAs or CIs.

A critical requirements for EnTK is to be able to handle failures at scale,
i.e., when both the probability and cost of failure increase. We consider
three main sources of failure: CI, task executables, and runtime systems. We
handle partial or transient failures of CI by restarting only the tasks
affected by the failure. The same approach is used for runtime failures while
task executable failures are returned to the user. Accordingly, EnTK
implements re-invoking failed entities, replication, redundancy, and graceful
termination.

Usability plays an important role in the development of EnTK, as it must meet
the aforementioned requirements for diverse programming and development
skills. Special attention was given to lowering the time to encode use cases
into executable distributed EBAs.

\jhanote{Qualitative + Quantitative please. i.e., try to capture
mean-time-to-failure or failure rates (accounting for
scale).}\mlnote{According to Youyi and Wenjie, the failure rate during the
summer was approx. 2 events every 25 events}

% Currently, use cases face a failure rate between 8 and 25~\% \vbnote{PU
% to confirm}. 


% \mtnote{Is this true only for when operating at scale? Is the importance of
% fault-tolerance is proportional to the scale?}\vbnote{Elaborated further.
% Please see.}.
% \mtnote{Sentences with multiple parenthetical clauses are difficult too
% follow and convey a sense of `heaviness' to the reader. I would
% iterate.}\vbnote{shortened, please see.}

% Currently, our use cases face a failure rate between 8-25~\% \vbnote{PU to
% confirm}. One of the most critical requirements for EnTK is to be able to
% handle failures when operating at scale. Both the probability and cost of
% failure increase with scale and hence it becomes increasingly important to
% handle failures.  The source of failures may be the CI, such as node or
% file-system failures, or application, such as segmentation faults, or
% underlying tools used by EnTK, such as connectivity timeouts or component
% failures. There are several methods of handling failures: re-invoking
% failed entities, replication, redundancy, and graceful termination.


% \mtnote{The focus here is on EnTK, not on its type of framework}\vbnote{
% agreed}
% \mtnote{or `ensemble applications', depending on who the first paragraph
% will be edited. Note that I did not use workflows because, as commented at
% the beginning of the subsection, I think we should minimize the association
% of EnTK to workflow systems.}\vbnote{agreed, fixed}


% The functionality and performance play an important role in the development
% of EnTK. Ease of learning and usage of the framework are fundamental
% because EnTK is designed and implemented specifically for domain scientists
% of diverse disciplines. The primary interest of the domain scientist lies
% in the development of various scientific applications and their results
% when deployed at scale and not in programming itself. Thus, the usability
% of the framework needs to be evaluated against the programming skills of
% the average end user with the goal of minimizing the time taken to encore
% the use cases into executable distributed EBAs.


% We collaborated with scientists from six research labs and
% diverse domains evaluating the usability of EnTK against different
% programming skills. Special attention was given to we devised ways to
% minimize the time taken to encode the use cases into executable distributed
% EBAs.


% ---------------------------------------------------------------------------
\subsection{Design}\label{ssec:design}

% \mtnote{Opening: Introduce layers and component linking them to the PST and
% C\&C models.}\vbnote{done, please see.}

% out only the information required downstream. Together, the these layers
% enable users to specify EBAs (PST model), convert user applications into
% EBA specifications that can then be executed on one or more CI by a chosen
% runtime system.

The design of EnTK is based on a model of EBAs called `PST' and a distributed
architecture. We use the PST model to enable users to describe and reason
about EBAs and the distributed architecture to abstract details and localize
information and functionalities to components.

\mtnote{I am not sure Task, Stage and Pipeline are
components.}\vbnote{fixed}\mtnote{Please note: objects are an implementation
detail. Here we are speaking at design level.}

% ------------
\subsubsection{PST Model} Implementations of EBAs share organizational
elements and patterns of dependencies among tasks. EBAs are a type of
workflow application with dependences among tasks, groups of tasks, or groups
of groups of tasks. These dependences may relate to the input and output data
of tasks but also to runtime evaluations, to the states of instruments or,
more generally, to any element that requires a barrier or a branch in the
control flow of the EBA\@.

On the base of these properties, we model EBAs by combining sets and lists:
\textit{Lists} represent the runtime dependences of tasks or groups of task;
\textit{sets} represent absence of dependences. We defined the following
user-facing constructs to express EBAs in terms of lists and sets:

\begin{itemize}
  \item \textbf{Task:} an abstraction of a computational task that contains
  information regarding an executable, its software environment and its data
  dependences.  
  % For the remainder of the paper, we use `Task' to refer to the EnTK Task
  % object.
  \item \textbf{Stage:} a set of Tasks without mutual dependences and that
  can be executed concurrently.
  \item \textbf{Pipeline:} a list of Stages where any stage \(i\) can be
  executed only after stage \(i-1\) has been executed.
\end{itemize}

Figure~\ref{fig:pst-model} shows an EBA described according to the PST model.
This application consists of a set of Pipelines, where each Pipeline consists
of a list of Stages, and each Stage consists of a set of Tasks. All the
pipelines can execute concurrently, all the states of each pipeline can
execute sequentially, and all the tasks of each stage can execute
concurrently.

\begin{figure}[t]
  \includegraphics[width=\columnwidth]{figures/entk_proposed_objects.pdf}
  \caption{Diagrammatic representation of an EBA consisting
          of a set of Pipelines with varying number of Stages. Each Stage has
          different number of Tasks.}\label{fig:pst-model}
\end{figure}


% \mtnote{What representation?}\vbnote{fixed}
% \mtnote{I would just introduce `barrier' as a fourth
% abstraction/notion/concept/object (?) alongside the other
% three.}\vbnote{Fixed, I would like to call it `concept' for now.}

% Although the PST model can express various EBAs, we identified the need to
% extend this representation to be able to express partial barriers between
% the various pipelines of the application when sets of pipelines need to be
% executed sequentially.

Note that this approach can be extended to Pipelines, describing EBAs with
dependences among groups of pipelines in terms of lists of sets of pipelines.
Further, the specification of branches in the execution flow of EBAs does not
require to alter the PST model: Branching events can be specified as tasks
where a decision is made about the runtime flow of the EBA\@. For example, a
task could be used to decide to skip some elements of a Stage, based on some
partial results of the ongoing computation.

% We will extend our current design to introduce both dependences among
% pipelines and branching in the next version of EnTK\@.

\mtnote{Definitions of workflow and workload should be now redundant. Note
how the given definition of workload is the same as the one of
Stage.}
%\paragraph{Working definitions}
% The application described via the PST model is interpreted and processed as
% `workflows' and `workloads' in the lower layers of EnTK\@. We define the
% two as follows:
% \begin{itemize}
%   \item \textbf{Workflow}: All Tasks of the application along with the
%   information of their dependencies and relative execution order.
%   \item \textbf{Workload}: Set of Tasks of the workflow whose dependencies
%   have been satisfied at a particular time and may be executed
%   concurrently.
% \end{itemize}


% ------------
\subsubsection{Architecture} EnTK sits between the user and the CI,
abstracting resource management and execution management from the end user.
Fig.~\ref{fig:entk-arch} shows the components (purple) and
subcomponents (green) of EnTK, organized in three layers: API, workflow
management, and task management.  

\jhanote{It is difficult to "see" these layers from the figure}\mtnote{See my
comment to the figure.}

\begin{figure}[t]
 \includegraphics[width=\columnwidth]{figures/entk_comm_model.pdf}
 \caption{EnTK communication model}\label{fig:entk-arch}\mtnote{This diagram
 needs to be iterated adding: layers on the right; numbers for the execution
 model description. Naming needs to be made consistent too.}
\end{figure}

% The Workflow Management layer exposes to the user the AppManager component
% to store the EBA description and information about available CIs. The
% AppManager initializes all the other components of EnTK and their
% communication infrastructure. The WF Processor component performs two
% operations: (i) identifies Tasks with satisfied dependencies, passing them
% to the Workload Management; and (ii) receives completed Tasks from the
% Workload Management, updating Task dependencies in the workflow.

The API layer enables users to describe EBAs in terms of pipelines, stages
and tasks. The Workflow Management layer retrieves information from the user
about available CIs, initializes EnTK, and holds the global state of the MBA
execution. The task management layer acquires resources via the runtime
system and uses them to execute EBA's tasks via the runtime system (RTS).

% \begin{figure}[t]
%  \includegraphics[width=\columnwidth]{figures/entk_design_translation.pdf}
%  \caption{EnTK architecture diagram. (Left) layer-based view; (right)
%  component-based view.}\label{fig:entk-architecture}
% \end{figure}

% The Resource Manager acquires resources via a runtime system. Currently,
% EnTK uses RADICAL-Pilot to submit pilots to HPC, HTC and Cloud resources,
% enabling late binding of pilots to resources and of tasks to pilots. The
% Execution Manager aggregates Tasks into a workload for concurrent
% execution, using information about Task requirements and available resource
% capabilities to make strategic decisions, possibly at runtime, on Task
% placement and execution.% \vbnote{sentence too long?}\mtnote{Better?}

The Workflow Management layer has two components: The AppManager and the WF
Processor. The AppManager uses a subcomponent called Synchronizer to update
the state of the EBA runtime. The WF Processor uses two subcomponents that
uses to queue and dequeue tasks from the Task Management layer: Enqueue and
Dequeue. The Task Management layer has one component, the Execution Manager,
that uses three subcomponents to acquire resources from the available CIs and
to execute the EBA's tasks on them: Emgr, RTS Callback, and heartbeat.

\jhanote{I'm also not sure that CI as a replacement for "resources" is
universally accepted. Generally: CI = software + hardware + peopleware.}

% Overall, EnTK requires users to provide EBA descriptions and a set of
% usable CIs. EnTK then converts EBA descriptions into workflows, analyzes
% the workflows for dependencies and creates workloads. Using information
% about the current state of the specified resources with the information
% about the application characteristics on these resources, a
% Task-to-resource mapping strategy is developed, according to which the
% Tasks of the workload are placed.

All the information on the state of the application execution is held by the
EBA description of the AppManager and all state updates of the execution
process are transactional. This makes EnTK fault-tolerant towards failures in
its components and subcomponents. Upon failure, each component can be
re-instantiated with minimal loss of information. In addition, the user may
also choose to enable resubmission of failed Tasks. When enabled, the dequeue
subcomponent reset the failed tasks to their initial state. These tasks are
then identified as new Tasks ready to be executed by the enqueue thread.

Another benefit of this architecture is the isolation of the RTS into a
stand-alone subsystem. This enables composability of EnTK with diverse RTS
and, depending on capabilities, multiple types of CIs. Further, EnTK assumes
the RTS to be a black box enabling fault tolerance for the whole RTS. When
the RTS fails or become unresponsive, EnTK can tear it down and bring it back
loosing only the Tasks that were in execution at the time of the failure.


% ------------
\subsubsection{Execution Model}

EnTK Components and subcomponents communicate and coordinate for the
execution of Tasks (blue). Users describe one or more EBA via the API,
instantiate the AppManager component with information about the available CIs
and then pass the EBA description to the AppManager for execution. The
AppManager holds the EBA description and, upon initialization, spawns the
Synchronizer, instantiates the WF Processor and Execution Manager, and
creates all the queues. The WF Processor instantiates Enqueue and Dequeue,
and the Execution Manager instantiates Emgr, RTS Callback, and Heartbeat.

% The following is the sequence of events that occurs in execution of a Task:
% \begin{enumerate}
%   \item Enqueue thread searches the workflow for Tasks that are ready to be
%   executed and pushes them to a `pending' queue.
%   \item Emgr thread pulls Tasks from the `pending' queue and executes them
%   via the RTS\@. Heartbeat thread constantly monitors if the emgr thread is
%   alive and responsive. The response indicates that execution is not
%   stalled due to possible errors in the RTS.
%   \item RTS callback thread pushes Tasks that have completed execution by
%   the RTS onto the `done' queue.
%   \item Dequeue thread pulls completed Tasks from the `done' queue and
%   updates the workflow based on the whether the Task failed or executed
%   successfully.
% \end{enumerate}

Once EnTK is fully initialized, WF Processor initiates the execution of the
EBA by creating a local copy of the EBA description from the AppManager and
tagging tasks for execution. Enqueue pushes these tasks to the Pending queue
(Fig.~\ref{fig:entk-arch}, 1). Emgr pulls tasks from the Pending queue
(Fig.~\ref{fig:entk-arch}, 2) and send them to the chosen RTS for execution
(Fig.~\ref{fig:entk-arch}, 3). RTS callback pushes tasks that have completed
execution by the RTS to the Done queue (Fig.~\ref{fig:entk-arch}, 4). Dequeue
pulls completed tasks (Fig.~\ref{fig:entk-arch}, 5) and tags them as done,
failed or canceled, depending on the return code of the RTS\@.


\jhanote{There is a problem with the figure. None of this is evident from the
figure as the numbers are missing}\mtnote{See my comment to the figure.}


Throughout the execution of the EBA, tasks, stages and pipelines undergo
multiple state transitions in both the WF Executor and the Execution Manager.
Each component and subcomponent synchronizes these transitions with the
AppManager by pushing messages through dedicated queues
((Fig.~\ref{fig:entk-arch}, 6). The AppManager pulls these messages and
updates the states of the EBA description. The AppManager then acknowledges
the updates via dedicated queues ((Fig.~\ref{fig:entk-arch}, 7). This
messaging mechanism ensures that the AppManager is always kept up to date
with any local changes and makes it the only stateful element of EnTK.

% stateless and with transactional operations. This design contributes to
% satisfy the requirement for fault-tolerance: stateless processes and
% threads are re-instantiated upon failure, without loosing any data produced
% by the tasks that have successfully completed.

% ---------------------------------------------------------------------------
\subsection{Implementation}\label{ssec:implementation}

% to keep the software footprint of EnTK small, existing tools, libraries and
% frameworks were used wherever possible. To be able to implement the above
% design, EnTK

% \begin{itemize}

% \item \textbf{Runtime system}: EnTK relies on a runtime system to manage
% task execution, data movement and resource management. One of the design
% objectives was to provide dynamic resource management, a type of which is
% to be able to execute more tasks than available resources would allow. EnTK
% achieves this via the use of Pilot-Job systems.

EnTK is implemented in Python, uses the RabbitMQ message queuing system and
the RADICAL-Pilot (RP) runtime system. All EnTK components are implemented as
processes and all the subcomponents as threads. AppManager is implemented as
a master process that spawns all the other processes. Tasks, stages and
pipelines are implemented as objects that are copied among processes and
threads via queues and transactions. Synchronization among processes is
achieved by message passing via queues.

% EnTK relies on the RabbitMQ messaging system to facilitate durable movement
% of this data. Our choice of RabbitMQ stems from its usability and
% functionality. RabbitMQ is a server-based message queuing (MQ) system that
% takes responsibility of setting up the entire messaging infrastructure on
% the machine without extensive manual involvement. Users are responsible for
% setting up RabbitMQ ‘queues’ to/from which messages can be pushed/pulled
% respectively.

EnTK relies on RabbitMQ to automate and manage the creation of the
communication infrastructure required by EnTK to copy objects and passing
messages among components. RabbitMQ provides methods to increase the
durability of messages in transit and of the queues, acknowledge messages
and, most importantly, it supports the requirement of managing at least
\(O(10^4)\) tasks concurrently. 

RabbitMQ is a server-based system and requires to be installed before the
execution of EnTK\@. This adds overheads but it also offers the following
benefits: (1) producers and consumers do not need to be topology aware
because they interact with the server; (2) messages are stored and can be
recovered upon failure of EnTK components; and (3) messages can be pushed and
pulled asynchronously because data can be buffered by the server upon
production.

% Pilot-Job systems provide placeholders or container jobs that are submitted
% to the target resource. These container jobs enable application-level
% scheduling of any number of executable units on these resources. Of the
% many pilot-systems currently developed, we select RADICAL-Pilot (RP). This
% is due to certain features unique to RP

% Note that EnTK is designed to be modular and extensible and therefore to be
% able to integrate with other general-purpose or special-purpose RTS\@. EnTK
% is actively developed and provides the necessary hooks for this coupling.

% \item \textbf{Message Queuing}: The communication model of EnTK consists of
%   multiple processes and threads that exchange data---both stateful objects
%   and synchronization messages---for the successful execution of an EBA.

Currently, EnTK uses RP as runtime system. RP is a pilot system that enables
late binding of tasks to resources. RP submits resource placeholders to one
or more CI to acquire resources. Once resources are acquires, RP executes a
software agent called `pilot'. This pulls tasks from the EBA and
schedules them on the acquired resources. In this way, users can execute
multiple tasks both concurrently and sequentially, depending on the amount of
available resources and their walltime. Compared to other pilot systems,
RP\@: (1) Supports MPI-based and GPU-based tasks; (2) offers extensive
profiling capabilities; and, (3) uses SAGA to support executions on HPC, HTC,
and Cloud CIs.

% In this section, we presented the requirements elicited from our use cases
% and the architecture and implementation of EnTK. We described the PST model
% that provides a uniform method to describe EBAs. The current runtime system
% used is RADICAL Pilot which uses SAGA for interoperability and hence makes
% EnTK usable on several heterogeneous CIs. The Pipeline, Stage, Task and the
% AppManager serve as the necessary abstractions that hide the complexity of
% task execution and resource management from the user. Lastly, through our
% current design choices of stateful and stateless entities along with our
% communication model, we account for component failures in EnTK and Task
% failures from the applications.

% \vbnote{I think we won't have space for the following. Might not be really
% necessary. Thoughts?}
% \paragraph*{API of the framework:} Add sample code snippet.

==> experiments.tex <==
We perform experiments to characterize the overheads in EnTK and its weak and
strong scaling performance. We then measure the overheads of EnTK when
executing, at scale, the implementation of the two use cases described
in~\S\ref{sec:use_cases}. 

\jhanote{"overheads in" EnTK vs "overheads of" EnTK. Same things or different overheads? If same, we should use "of" EnTK}

We use four applications in our experiments: Sleep,
Gromacs~\cite{abraham2015gromacs}, Specfem~\cite{komatitsch2002spectral}, and
Canalogs~\cite{alessandrini2015analog}. Sleep and Gromacs enable the control 
of the duration of task execution and to compare EnTK overheads across task
executables. Gromacs and the NTL9 protein offer a reference benchmark for
EnTK weak and strong scalability, while Specfem and Canalogs are required by
the two use cases of this paper. \jhanote{not sure what, "Gromacs and the NTL9 protein offer a reference benchmark" means?}

We perform our experiments on four CIs: XSEDE SuperMIC, Stampede, Comet and
ORNL Titan. We use four resources for the characterization of EnTK overheads;
Titan for the characterization of the scalability; and Titan and SuperMIC for
the use case implementations. \jhanote{Not sure what "use case"
implementations means?}


% ---------------------------------------------------------------------------
\subsection{Characterization of EnTK Performance}\label{ssec:entk_validation}

We use a prototype of EnTK to benchmark its performance, providing a
reference hardware configuration to support execution of up to \(O(10^6)\)
tasks. We then perform four experiments to characterize the overheads of
EnTK\@.

% ------------
\subsubsection{Performance of EnTK Prototype}

We prototyped the most computationally expensive functionality of EnTK to
instantiate multiple producers and consumers of tasks. Each producer pushes
tasks into RabbitMQ queues and each consumer pulls tasks from these queues,
passing them to an empty RTS module.
% The prototype abstracts RTS implementations and most of the architectural
% details described in~\S\ref{ssec:design} but implements the most
% computationally expensive functionality of EnTK to manage tasks.
We benchmarked configurations with \(10^6\) tasks and a different number of
producers, consumers, and queues, measuring: producers and consumers time,
total execution time, base memory consumption when the components are
instantiated, and peak memory consumption during the execution.

\begin{figure}[t]
  \includegraphics[width=\columnwidth]{figures/prototype_perf.pdf}
  \caption{Execution time and memory consumed by EnTK prototype with multiple
  producers and consumers when processing \(10^6\)
  tasks.}\label{fig:entk_prototype_perf}
\end{figure}

Fig.~\ref{fig:entk_prototype_perf} shows that tuning of the prototype can
reduce the processing time linearly, at the cost of increased memory usage.
Eight producers and consumers require 107 seconds to process \(10^6\) tasks,
with a peak memory consumption of 3,126MB\@. Uneven distributions of
producers and consumers resulted in lower efficiencies than when using even
distributions.

The execution model of EnTK can be tuned on the basis of this benchmark,
workload requirements, and hardware capabilities. This benchmark shows that
the performance of the core functionality of EnTK depends on the number of
tasks that are processed concurrently. This has relevant implications for the
understanding of EnTK overheads and scalability.

% ------------
\subsubsection{Overheads}

\vbnote{Reviewer 2, Q4: It looks to me like it should be: the individual 
overheads, the overall scalability, and finally the use with real
applications. For overheads, that would be the current Figure 6, though maybe
the experiments should be run on multiple platforms (Figure 8). The
importance of individual overheads needs to be explained in terms of their
influence on the rest of the system (the CPU consumption, the (in)ability of
the framework to perform other functions during lengthy setup/teardown
phases, etc). Why is there so much focus on EnTK Management Overhead but not
on other overheads? }

% Execution of an application using EnTK involves 92 events, including
% validation of the application and of the resource descriptions, submission
% of resource request, creation of tasks, and translation of tasks to and
% from the RTS\@.
We designed four experiments to characterize the overhead added by EnTK to
the time taken to execute an application, excluding the time taken by the
resources to become available. We characterize EnTK overhead against four
parameters that are likely to vary among applications: Task executable; task
duration; CI on which the application is executed; and structure of the
application, i.e., the way in which tasks are grouped into stages and stages
into pipelines.
% Accordingly, we performed four experiments where we measured the overhead
% of EnTK for each one of these parameters. We decomposed the total runtime
% into several time components, measuring the dominant overheads of EnTK and
% RTS, the total data staging time, and the total task execution time:
We measured the overheads that dominate EnTK and RTS runtime alongside the
total task execution time and, when required, the total data staging time:

\begin{itemize}
    \item \textbf{EnTK Setup Overhead}: Time taken to setup the messaging
    infrastructure, instantiate all the components and subcomponents, and
    validate the application and resource descriptions.
    \item \textbf{EnTK Management Overhead}: Time taken to process the
    application, translate tasks from and to RTS-specific objects, and
    communicate pipelines, stages, tasks and control messages.
    \item \textbf{EnTK Tear-Down Overhead}: Time taken to cancel all EnTK
    components and subcomponents, and shutdown the messaging infrastructure.
    \item \textbf{RTS Overhead}: Time taken by the RTS to submit and manage
    the execution of the tasks.
    \item \textbf{RTS Tear-Down Overhead}: Time taken by the RTS to cancel
    its components and to shutdown.
    \item \textbf{Data Staging Duration}: Time taken to copy data between
    tasks using the functionality available on the resource (in this case,
    the Unix POSIX \texttt{cp} command).
    \item \textbf{Task Execution Time}: Time taken by the task executables to
    run on the CI\@.
\end{itemize}

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=\textwidth]{figures/entk_all_overheads_unified.pdf}
    \caption{Overheads and Task Execution Time as function of (a) Task
             Executable, (b) Task Duration (c) Computing Infrastructure (d)
             Application Structure}\label{fig:overheads}
\end{figure*}


% ------------
% Experiment 1
% ------------
\paragraph*{\textbf{Experiment 1: Task Executable}} We run two applications
on the XSEDE SuperMIC cluster, each with 1 pipeline, 1 stage per pipeline, 16
tasks per stage. The first application runs the Gromacs \texttt{mdrun} task
executable; the second the \texttt{sleep} executable. The execution time of
each task is set to \(\approx\)250 seconds. We measure Task Execution Time,
Data Staging Duration, and the EnTK and RTS overheads as defined above.

Fig.~\ref{fig:overheads}a shows that EnTK Setup Overhead is negligible for
both task executables. This overhead depends on the performance of the
machine on which EnTK is executed and should vary
% , not on the type of workload managed or on the RTS used for its execution.
across Experiments 1--4 only when the host machines changes.

EnTK Management Overhead has an almost identical value for the two task
executables. This is consistent with a core element of EnTK design:
decoupling task management from task execution. EnTK manages tasks until they
are passed on to the RTS, playing no role in their actual execution. This
contributes to the portability of EnTK across diverse scientific domains and
CIs.

We attribute the variations of EnTK Tear-Down Overhead and of RTS Tear-Down
Overhead to the time taken by Python to terminate processes and threads.
Across Experiments 1--4, we observe Python taking variable amount of time to
cancel processes and threads, with values between \(\approx\)1 and
\(\approx\)10s for EnTK Tear-Down Overhead and \(\approx\)3 and
\(\approx\)80s for RTS Tear-Down Overhead. This is expected as the RP RTS
uses significantly more processes and threads than EnTK leading to higher
average termination time.

We explain the variation of RTS Execution Overhead by noticing that, at runtime, RP initiates communications between the CI and a remote database,
and reads and writes to the shared file system of the CI to create the
execution environment of each task. Further, RP uses different tools to
distribute the execution of tasks across multiple compute nodes---e.g.,
\texttt{aprun} and \texttt{openmpi}. 

We expect RTS Execution Overhead to vary across Experiments 1--4 but a
detailed analysis of the interplay among network latency, I/O performance,
and the performance of third party tools and libraries is beyond the scope of
this paper. This is consistent with EnTK design: the RTS (e.g., RP in this
case) is assumed to be a blackbox.

Data Staging Duration is sub-second for \texttt{mdrun} as only few files, of
O(KB) size each, are copied between tasks using file-system capabilities. No
data are stages for \texttt{sleep}.

% As described in~\S\ref{sec:entk}, EnTK is designed to be decoupled from the
% RTS\@. As such, the following experiments characterize the overheads of
% EnTK, independent from those of the RTS\@. We focus on the EnTK Management
% Overhead because EnTK Setup Overhead, given the same host machine where
% EnTK is run, is similar for every application and measured to be
% negligible. EnTK Tear-Down Overhead depends on Python and, while it affects
% the execution time of the application, it does not depend on the
% architecture of EnTK\@.

% RTS overhead is specific to RP and independent of EnTK\@. RTS tear-down
% overhead is RP specific as well and mostly determined by Python thread and
% process termination durations similar to those measured for EnTK\@. We plot
% the overheads in the remainder of the experiments but we discuss them only
% when they show a peculiar behavior.

% ------------
% Experiment 2
% ------------
\paragraph*{\textbf{Experiment 2: Task Duration}} We run four applications on
the XSEDE SuperMIC cluster, each with 1 pipeline, 1 stage per pipeline, 16
tasks per stage and with the \texttt{sleep} task executable and no data
staging. The four applications vary for the duration of task execution: 1,
10, 100, and 1000 seconds. 
% We measure EnTK Management Overhead and Task Execution Time.
Fig.~\ref{fig:overheads}b shows that Task Execution Time grows with the
duration of the \texttt{sleep} command. EnTK and RTS overheads measures are
consistent with what already observed in Experiment 1, showing that their
values do not significantly depend on the duration of the tasks executed.

% . As in Experiment 1, EnTK Setup Overhead and EnTK Management Overhead
% remain stable at around 0.1s and 10s respectively. EnTK Tear-Down Overhead
% is on average \(\approx\)5s, while RTS overheads are consistent with
% already observed.

% As with Experiment 1, the almost linear behavior of EnTK Management
% Overhead is explained by the decoupling between EnTK and task executables:
% once tasks are handed over to the RTS, EnTK waits for their exit code,
% accumulating no further overhead.

% ------------
% Experiment 3
% ------------
\paragraph*{\textbf{Experiment 3: Computing Infrastructure (CI)}} We run one
application on four resources: XSEDE SuperMIC, Stampede, Comet and ORNL
Titan. The application has 1 pipeline, 1 stage per pipeline, 16 tasks per
stage and the task executable \texttt{sleep} executes for 100 seconds with no
data staged.

Fig.~\ref{fig:overheads}c shows that, as per experiment design, Task
Execution Time is 100 seconds on all four CIs. EnTK Management Overhead is
\(\approx\)10 seconds on SuperMIC, Stampede and Comet, and \(\approx\)2
seconds on Titan. We attribute this difference to the host on which EnTK was
executed: a virtual machine (VM) hosted at TACC for the applications executed
on the XSEDE clusters, an ORNL login node for those executed on Titan. This
is consistent with the performance characterization in
Fig.~\ref{fig:entk_prototype_perf} and with EnTK design: Application
management is performed on the user host while task execution on the target
CI\@.

% EnTK avoids running system software on HPC login nodes when policies do not
% allow it.
EnTK Setup Overhead is smaller on Titan due to the login node being faster
than the hosted VM\@. EnTK and RTS Tear-Down overheads differ between Titan
login node and the hosted VM due to different Python deployments. RTS
Overhead varies according to what explained in Experiment 1.

% ------------
% Experiment 4
% ------------
\paragraph*{\textbf{Experiment 4: Application Structure}} 
% In experiments 1--3, we used the same structure for all the applications,
% i.e., 1 pipeline, 1 stage per pipeline, 16 tasks per stage. In this
% experiment, we
We run applications with three different structures on XSEDE SuperMIC\@: (1)
16 pipelines, 1 stage per pipeline, 1 task per stage; (2) 1 pipeline, 16
stages per pipeline, 1 task per stage; and (3) 1 pipeline, 1 stage per
pipeline, 16 tasks per stage. The task executable \texttt{sleep} executes for
100 seconds in all the applications without data staging. We use application
\#3 as baseline for comparison with the previous three experiments, and we
measure EnTK Management Overhead and Task Execution Time.

Fig.~\ref{fig:overheads}d shows that with 16 pipelines (first) and 16 tasks
(last), all the tasks execute concurrently and hence Task Execution Time is
\(\approx\)100 seconds. However, with 16 stages, tasks execute sequentially,
resulting in Task Execution Time of \(\approx\)1600 seconds. 
% Although Task Execution Time varies depending on the structure of the
% application,
EnTK Management Overhead is stable at \(\approx\)10 seconds. This is
consistent with the results of the previous experiments and the decoupling
between task management and execution.

EnTK Setup Overhead and RTS Tear-down Overhead are consistent with what
already observed but RTS Overhead grows proportionally to Task Execution
Time when using 16 stages. This is explained by considering the reduced
concurrency of all time components of RTS Overhead: When executing tasks
sequentially, the overhead accumulated for each task adds to the total RTS
Overhead time.

% -----------------------
% Summary Experiments 1-4
% -----------------------
\paragraph*{\textbf{Summary Experiments 1--4}} EnTK setup, management, and
tear-down overheads do not sensibly vary with the four parameters of task
execution we measured. Setup and management overheads depend on the memory
and CPU performance of the host on which EnTK is executed, while the
tear-down overhead on the Python version utilized. This validates our design
and implementation against our requirements for a toolkit that can be used in
various scientific domains and with different task executables across
heterogeneous CIs.

\mtnote{Addresses reviewer comment about Python.}

In absolute terms, EnTK overheads are between \(\approx\)10 and 20 seconds,
becoming relevant only when considering corner cases in which applications
have second-long tasks to execute. Experiment 3 shows that also these corner
cases could be handled by running EnTK on a host with a suitable amount of
resources. RP RTS shows overheads up to \(\approx\)80s, confirming the
limitations to applications with at least minutes-long tasks. EnTK and RP
should be coded, at least partially, in a different language to manage the
execution of minute- and seconds-long ensembles.

% Python's termination of processes and threads accounts for  for large part
% of the overheads we measured in these experiments. Both EnTK and RTS
% tear-down overheads amount to never more than \(\approx\)80s and, most of
% the times, are between 10 and 20s. This makes EnTK and RP a viable options
% for managing tasks that executes for few minutes and beyond. EnTK and RP
% should be coded, at least partially, in a different language to manage the
% execution of minute- and seconds-long ensembles.

% ---------------------------------------------------------------------------
\subsection{Scalability}

We perform two experiments to characterize weak and strong scalability of
EnTK\@. As with Experiment 1--4, we measure and compare all overheads, Data
Staging Duration and Task Execution Time. Weak scaling relates these measures
to the amount of concurrency used to execute the application's tasks; Strong
scaling to the amount of serialization. 

% Experiments 1--4 shows that measuring EnTK overheads isolates EnTK
% performance.

% ------------
\subsubsection{Weak scalability}

For the weak scaling experiment,
% measures EnTK Management Overhead and Task Execution Time maintaining
% maintains constant the ratio between number of tasks and number of
% available cores. In this way, the application's tasks are executed with
% maximum concurrency. We
we run seven applications on Titan, each with 1 pipeline, 1 stage per
pipeline, and 64, 128, 256, 512, 1024, 2048, and 4096 tasks per stage. Each
task executable is Gromacs \texttt{mdrun}, configured to use 1 core and
execute for \(\approx\)600 seconds. The total amount of cores acquired is
equal to the number of the application's tasks. \mtnote{wait for Vivek's details on data staged.}
% As with the strong scaling experiment, the design of these experiments is
% based on the requirements of the two use cases of this paper.

\begin{figure}[t]
  \includegraphics[width=\columnwidth]{figures/weak_scaling_titan_orte.pdf}
  \caption{Weak scalability on Titan: 64, 128, 256, 512, 1024, 2048, and 4096
  1-core tasks executed on the same amount of cores. 
  % Task Execution Time is constant up to 1024 tasks/cores but increases
  % super-linearly up to 4096 tasks. EnTK Management Overhead is constant up
  % to 2048 tasks but then increases linearly with the number of
  % tasks.
  }\label{fig:weak_scaling}
\end{figure}

Fig.~\ref{fig:weak_scaling} shows that the Task Execution Time remains
constant up to 1024 tasks/cores but then increases gradually by 100 seconds
up to 4096. Analysis of the RTS profiles shows that this behavior is due to
delays in the Executor module of the RTS Agent. Ref.~\cite{rp-paper-isc}
offers a detailed characterization of these delays and their causes.

EnTK Management Overhead remains constant till 2048 tasks as the number of
tasks are too small to cause a variation. The overhead, then, increases
linearly between 2048 and 4096 tasks: With the increase of the number of
concurrent tasks, EnTK requires more resources and starts to strain the
resources of the host on which it is executed. The other EnTK and RTS overheads appear consistent with what already noted in Experiments 1--4. 

% This is consistent with what observed in the Strong scaling experiment,
% where EnTK had to manage only 512 concurrent tasks and with
% Fig.~\ref{fig:entk_prototype_perf}.

We recorded Data Staging Duration for runs with between 512 and 4096 tasks
(data for runs with 64 and 256 tasks were corrupted). Data staging is
performed \mtnote{wait for Vivek's details on data staged.}. The time taken
to stage input and output files grows linearly with the number of tasks
executed: from \(\approx\)11s with 512 tasks to \(\approx\)88s with 4096
tasks. As this time depends on the performance of Titan shared file system
and the \texttt{cp} command, a less linear behavior is expected with larger
(amount of) files.

% ------------
\subsubsection{Strong scalability}

\vbnote{Reviewer 2 recommended rerunning strong scaling experiments with
constant workload and varying resources}

For the strong scaling experiment, 
% measures EnTK Management Overhead and Task Execution Time by increasing the
% number of cores used to execute a constant number of tasks. We
we run four applications on Titan, each with 1 pipeline, 1 stage per
pipeline, 8192 tasks per stage and a total of 1024, 2048 and 4096 cores. Each
task executable is Gromacs \texttt{mdrun}, configured to use 1 core and
execute for \(\approx\)600 seconds. In this way, we execute at least 2
generations, each with 4096 tasks, within the 2 hours walltime imposed by
Titan's queuing policies. \mtnote{wait for Vivek's details on data staged.}

% We designed this experiment based on the upper bound on the weak scaling
% experiment and job policies on ORNL Titan. We set the upper bound of the
% number of cores same as that of the weak scaling experiment, i.e. 4096
% cores. The scheduling policy on Titan mandates that all jobs using less
% than 2048 cores have a maximum walltime of 2 hours. In accordance with the
% same, we determined that 8192 tasks and a lower bound of 1024 cores can be
% used.

\begin{figure}[t]
  \includegraphics[width=\columnwidth]{figures/strong_scaling_titan_orte.pdf}
  \caption{Strong scalability on Titan: 8192 1-core tasks
  are executed on 1024, 2048 and 4096 cores. 
  % Task Execution Time reduces linearly with increasing the number of cores.
  % EnTK Management Overhead is consistently \(\approx\)2
  % seconds.
  }\label{fig:strong_scaling}
\end{figure}

Fig.~\ref{fig:strong_scaling} shows that Task Execution Time reduces linearly
with increase in the number of cores. The availability of more resources for
the fixed number of tasks explains this linear reduction in the Task
Execution Time. EnTK Management Overhead is between \(\approx\)8 and 10s,
confirming what already observed in the previous experiments. The slight
improvement in the performance is due to some optimization of EnTK code
performed for this experiment.

All the other overheads and Data Staging Duration remain constant across the
experiment runs. This suggests that both EnTK and RP overheads mostly depends
on the number of managed tasks, not on the size of the pilot on which they
are executed. This is confirmed for RP in Ref.~\cite{rp-paper-isc}.

Fig.~\ref{fig:entk_prototype_perf} shows that EnTK can be configured to
execute \(10^{6}\) tasks in less than 200 seconds and consuming less than 4GB
of memory. Extrapolating and accounting for a faster CPU on Titan's login
nodes, EnTK should manage enough tasks to fill all of Titan cores with an
overhead of less than 50 seconds.


% ---------------------------------------------------------------------------
\subsection{Use Cases at Scale}

We implement and execute at scale the most computationally intensive and
fault-prone step of the tomography workflow, and the full adaptive analog
workflow (\S\ref{sec:use_cases}) with EnTK.

% ------------
\subsubsection{Seismic inversion }\label{ssec:exp_seismic}

We use EnTK to encode the forward simulations of the seismic tomography
workflow described in~\S\ref{ssec:seismic_inversion} and depicted in
Fig.~\ref{fig:use_case_tomo_wf}. These simulations account for more than 90\%
of the total computation time of the current implementation of the workflow,
requiring 384 nodes for each earthquake simulation. When earthquakes are
concurrently simulated, they require a sizable portion of Titan and incur a
high rate of failures. Without EnTK, these failures result in manual
resubmission of computations, adding a significant overhead due to queue wait
time on user intervention.

We characterize the scalability of forward simulations with EnTK by running
experiments with a varying number of tasks, where each task uses 384
nodes/6144 cores to forward simulate one earthquake. Understanding this
scaling behavior contributes to optimize the execution of the whole workflow,
both by limiting failure and enabling fault-tolerance without manual
intervention. Ultimately, this will result in an increase of the overall
efficiency of resource utilization and in a reduction of the time to
completion.

The current implementation of forward simulations causes heavy I/O on a
shared file system (\S\ref{ssec:seismic_inversion}). This overloads the file
system, inducing crashes or requiring termination of the simulations. EnTK
and RP utilize pilots to sequentialize a subset of the simulations, reducing
the concurrency of their execution and without having to go through Titan's
queue multiple times. This is done by reducing the number of cores and
increasing the walltime requested for the pilot.

Fig.~\ref{fig:specfem_concurrency} shows that increasing concurrency leads to
a linear reduction of Task Execution Time, with a minimum of \(\approx\)180
seconds. Interestingly, reducing concurrency eliminates failures: we
encountered no failures in executions with up to \(2^4\) concurrent tasks and
6144 nodes. At \(2^5\) concurrent tasks and 12288 nodes, 50\% of the tasks
failed due to runtime issues.

\begin{figure}[t]
  \includegraphics[width=\columnwidth]{figures/specfem_exec_time_varying_concurrency_titan.pdf}
  \caption{Task Execution Time of forward simulations using EnTK at
  various values of concurrency. The total number of earthquakes simulated
  varies as 1, 2, 4, 8, 16 and 32 where each earthquake maps to a unique
  task. }\label{fig:specfem_concurrency}
\end{figure}

EnTK automatically resubmitted failed tasks until they were successfully
executed. In the run with \(2^5\) tasks, EnTK attempted to run a total of 157
tasks. The resulting Task Execution Time was \(\approx\)360 seconds, similar
to that of a run with with \(2^4\) concurrent tasks
(Fig.~\ref{fig:specfem_concurrency}).

EnTK and RP enable reasoning and benchmarking the concurrency of an execution
without any change in the executable code. This gives insight on how to
tailor a given computational campaign on a specific CI\@. The insight gained
via our experiments can be immediately used in production: On Titan, forward
simulations are best executed with \(2^4\) concurrent tasks. Further,
fault-tolerance has an immediate impact on production runs, eliminating one
of the most limiting factor of the previous implementation of the workflow.

% ------------
\subsubsection{Meteorological Probabilistic Forecasts}

We use EnTK to implement the \gls{AUA} algorithm to iteratively and
dynamically identify locations of the analogs. We also implement the
\textit{status quo} method of generating these analogs, i.e., random
selection of locations in each iteration. We perform experiments to compare
the two implementations and observe the speedup of the proposed algorithm. We
repeat the experiment 30 times for statistical accuracy, initializing both
implementations using the same initial random locations.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/EX_PSU_error_plot_2x2.pdf}
    \caption{Predictions from random and adaptive methods. (a) theoretical
    true value, (b) the interpolated map from 1800 randomly picked locations,
    (c) the interpolated map from 1800 locations identified using AUA, (d)
    box plots of the errors for both
    implementations}\label{fig:psu-error-plot}
\end{figure}

Fig.~\ref{fig:psu-error-plot} shows the prediction maps and errors obtained
from the two implementations. With 1800 locations calculated for both
prediction maps (Fig.~\ref{fig:psu-error-plot}(b),
Fig.~\ref{fig:psu-error-plot}(c)), the \gls{AUA} algorithm generates a map
with certain areas that have a better representation of the analysis than the
map generated by a random selection of pixels.

The box plot in Fig.~\ref{fig:psu-error-plot}(d) shows the distribution of
the errors for the two implementations. The error converges faster in the
\gls{AUA} algorithm than in the random selection. The total amount of
potential locations (pixels) is 262972; thus both implementations use a small
fraction of the available locations but the \gls{AUA} algorithm is
automatically steering the computation at each iteration. EnTK and RP avoid
the usual shortcoming of this approach: The evaluation required by the
steering can be implemented as a task and iterations do not wait in the HPC
queue, even if their number is unknown before execution. These results
suggest that the \gls{AUA} algorithm over random selection of points is well
suited for very large domains.

==> use_cases.tex <==
We describe the two use cases of this paper, focusing on their computational
and functional requirements.

\subsection{Seismic Inversion}\label{ssec:seismic_inversion}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% High level problem overview
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
A number of seismic algorithms have been developed to improve the
understanding of the Earth's interior. In what follows, the focus is on the
most powerful of these techniques: the inversion of full-waveform,
wide-bandwidth seismic data~\cite{Virieux2009}. Scaling full waveform
inversion to larger models~\cite{BozdagEtAl2016} and the assimilation of data
from thousands of earthquakes is challenging, not only by the amount of
computational resources it requires, but also by the quantity of human labor
needed to perform such studies. These challenges mandate a more automated
approach such as the one implemented by the EnTK\@.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% High level workflow overview
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
A brief overview of the scientific workflow involved to perform seismic
tomography is useful to understand where the challenges lie. For clarity
purpose, we restrict the discussion to global tomography; where the models
are approximations of the entire Earth's structure and where data are
seismograms recording earthquake generated waves. A high level view of this
workflow is shown in Figure~\ref{fig:use_case_tomo_wf}. Seismic data (or
seismograms) are recorded as time series of a physical quantity, such as
displacement, velocity, acceleration or pressure. The overall goal is to
iteratively minimize differences between a set of observed data and
corresponding synthetic data through a pre-defined misfit function. As the
adjoint-based optimization procedure is carried on and the data misfit
decreases, the model get closer to reality.

% A typical seismic waveform tomography workflow is shown on
% Figure~\ref{fig:use_case_tomo_wf} and consists of three major steps: (1)
% numerical simulations of forward and adjoint wavefields, (2)
% pre-processing, and (3) post-processing. Each of these steps involve
% several moving parts.

\begin{figure}[t] %  figure placement: here, top, bottom, or page
   \centering
   \includegraphics[width=\columnwidth]{figures/use_case_tomo_workflow_pst.pdf} 
   \caption{Simplified seismic tomography workflow. This iterative process
   consists in 5 steps. (1) For each earthquake, synthetic data are
   generated, (2) both synthetic and real data are processed and compared to
   create the so called adjoint sources that are then (3) used to initiate
   adjoint simulations. (4) The kernels obtained for each earthquake
   are them summed to produce a gradient to be used (5) the optimization and
   the update routines. This process is repeated until
   convergence.}\label{fig:use_case_tomo_wf}
\end{figure}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Computational characteristics 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The computational characteristics of each part of the workflow are better
explained by looking at the specificities of state-of-the-art production
runs. As of today, and at the global scale, routine production work consists
in assimilating data from about a thousand earthquakes. The simulations (both
forward (1) and adjoint (3)) are by far the most computationally expensive
part and each of them is ran on 384 GPUs for a total of 10~millions
core-hours per iteration. The data processing part (2) is relatively
inexpensive, utilizing about 48000 core-hours in each iteration but requiring
the data to undergo a significant number of steps. The post-processing (4)
takes about 10000 core-hours, in which smoothing the kernels is the most
time-consuming part. The optimization (5) takes about 1 million core-hours,
since forward simulations of a subset of events are launched to determine the
step length.


% \mlnote{Wenjie: how expensive are parts (4) and (5)?}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Challenges: scalability, reliability, usability, ...
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Each part of the workflow has been relying on a Python-based proto-workflow
management system using abstractions provided by the RADICAL-SAGA package.
However, scaling to higher resolutions and assimilating data from a complete
database of 6,000 recorded earthquakes requires a paradigm shift and the
adoption of a more automated approach to ensure reliability, minimize errors
at the user level and lower the overall time to solution.

From a workflow management point of view, several challenges are provided by
this seismic tomography workflow. First, it interleaves relatively large
simulations with smaller data-processing tasks, or each task requiring
respectively leadership-scale systems and moderately sized clusters. Second,
it is coupled with a data management problem, since some data needs to be
temporarily or permanently saved, or moved around. \mlnote{Rutgers: why did
you picked this particular problem?}\mtnote{Does it work?}

Ensemble-based applications are particularly well-suited to encode the
seismic tomography workflow. In EnTK, both the simulation and analysis phases
can be described as stages of a pipeline, avoiding the need for a dedicated
MPI application to execute multiple simulation concurrently. EnTK also allows
the execution of the ensemble of simulations with a varying degree of
concurrency and sequentiality, without requiring specific coding. EnTK offers
automation and fault-tolerance avoiding the overheads experienced by the
users with full-fledged workflow systems.


% ---------------------------------------------------------------------------
\subsection{High Resolution Meteorological Probabilistic Forecasts}\label{ssec:anen}

% \jhanote{measure success at: (i) adaptivity, and (ii) large size/scale, and
% ``automation''.}
% \jhanote{on scale: can we ``reach a limit on return on investment on
% computing \# of pixels''!}

%\footnote{\url{https://docs.google.com/document/d/1kxX0sucCNJtbjAONr-yP4JtLz
%7KhOmj9wqATPM8kO3w/edit}}

%The goal of the second science driver is to quantify the \gls{PV} energy
%potential over all regions of the USA based on historical observations and
%future possible climate scenarios. The vision is to create the energy smart
%grid of the future that includes a significant fraction of renewable energy
%generation. Understanding the potential of \gls{PV} power generation under
%different climate scenarios is paramount to build sustainable solutions to
%use renewable energy to satisfy future energy demands.

% ------------
%\subsubsection*{Analog Ensemble}

We used a new methodology called \gls{AnEn}~\cite{anen} to generate
high-resolution, probabilistic forecasts for specific parameters like
temperature or cloud cover. 
% starting from a deterministic future forecast. %These high resolution
% variable fields are input to a \gls{PV} model to estimate the amount of
% power generated \cite{cervone2017short, alessandrini2015analog}.
We developed a specific implementation of \gls{AnEn} to generate
high-resolution depictions of environmental variables, using relationships
between current and past forecasts from the \gls{WRF} data. To generate an
analog ensemble for a given time \(t\) and a given location \(l\), our
implementation finds the most similar historical forecasts within the search
space based on a similarity metric.
% To generate an analog ensemble for a given time \(t\) and a given location
% \(l\), the most similar historical forecasts will be found within the
% search space based on a similarity metric.
The observations associated with the most similar past forecasts are used as
analogs. These observations can be calibrated using spatio-temporal
coefficients if predictable errors are known (e.g., the degradation of a
solar panel yields lower wattage as a function of time).

We drove the development and assessed the suitability of EnTK for analog
computation by testing the \gls{AnEn} method with dataset including forecast
predictions for 13 variables (e.g., wind speed, precipitation, pressure,
etc.) for the years 2015 and 2016. Data for both analysis and forecasts are
from the \gls{NAM} maintained at the \gls{NCAR}.

One of the challenges of this use case is that analogs have to be computed
for a large number of geographical locations, potentially including millions
of specific locations. However, in principle it is possible to exploit some
unique physical characteristics of the predictand variable (e.g.,
temperature), and make assumptions that can drastically decrease the amount
of computations needed while maintaining the prediction accuracy.

% For example, temperature tends to vary smoothly between adjacent grids,
% except for cases with drastic changes in orography, land cover type, or the
% atmospheric circulation.

% ------------
%\subsubsection*{Adaptive Unstructured Analog Algorithm}

%The \gls{AnEn} is a computationally intensive but highly parallelizable and scalable technique to generate probabilistic forecasts. Therefore, this method is well-suited to high-performance computing environment.

%When deploying the \gls{AnEn} method on supercomputers, it is possible to optimize the allocation of tasks by dedicating more resources to locations where higher spatial resolution is needed. 

In this particular application, the simplest scenario is to compute analogs
at each grid point. This solution yields the highest possible resolution, but
it is very slow and most importantly, often unnecessary. In fact, for some
output variables, such as temperature, the highest resolution of the analogs
is required only at specific regions, where drastic gradient changes occur.
Therefore, we implemented a dynamic iterative search process, named the \gls{AUA} algorithm,
which generates analogs at specific points, and interpolates the analogs using an
unstructured grid.

%One of the main difficulties with this approach is that the algorithm is
%iterative and at each iteration it performs a variable number of operations.
%%\jhanote{Suggestion: We could zap from here...} 
%%If the resource allocation is fixed, the distribution of computation across nodes and cores is likely not optimal.
%Furthermore, our approach requires resource management, which by
%itself is a difficult and time consuming process that takes scientists
%away from the science.
%%Optimizing the allocation of resources has also the added benefit of minimizing queue wait time.
%Without a proper job management, when the algorithm performs
%a queuing request at each iteration, the jobs might spend more time waiting to be
%executed, than the execution time itself. If the algorithms allocates all
%resources at once, more resources than those strictly needed might be
%allocated, again leading to longer queue wait time. 
%
%EnTK, serving as a middleware between the \gls{AnEn} and supercomputers,
%enables us to design an algorithm, named the \gls{AUA} algorithm, that takes
%the full advantage of dynamically allocating tasks without having to allocate
%resources and submitting queue requests. EnTK helps users to keep the job
%session alive to avoid submitting multiple jobs; and by using an iterative
%approach, the algorithm can generate higher predictions for places where
%there is higher variability, using an unstructured grid. EnTK also empowers
%us to achieve a higher level of automation where the algorithm can allocate
%more computing resources when a larger search space is required in order to
%improve prediction accuracy. This is paramount when not many good analogs
%are found in the previous search space.
%%Finally, EnTK takes cares of the job management, allowing the algorithm to be deployed on different supercomputers without having to learn and adapt to different job submission processes.
%%\jhanote{...to here.}

%\jhanote{proposed alternative}

One of the main difficulties with this approach is that the algorithm is
iterative, and at each iteration it performs a variable number of operations.
EnTK addresses the resource management challenges arising from such
variations: by using an iterative approach, the algorithm can generate higher
predictions for places where there is higher variability, using an
unstructured grid. EnTK also empowers us to achieve a higher level of
automation where the algorithm can allocate more computing resources when a
larger search space is required in order to improve prediction accuracy. This
is paramount when not many good analogs are found in the previous search
space.

%\jhanote{Possibly zap from here... } Figure~\ref{fig:psu-use-case} shows the
%workflow of the \gls{AUA} algorithm. The \gls{AUA} algorithm is developed to
%take the advantage of EnTK's ability to dynamically manage computation
%resources and to allocate ensemble tasks to the available nodes. The
%workflow can be divided into 4 steps: initialization, preprocessing,
%iterative computation, and post-processing.
%
%
%The initialization step specifies the starting parameters for \gls{AnEn} and
%EnTK\@. For \gls{AnEn}, it specifies the search space and the test space to
%generate the predictions, together with the extra arguments for the
%algorithm; for the EnTK, the initialization step specifies the supercomputer
%environment and the initial amount of computing resources to use for
%execution. The preprocessing step generates preparatory data that will be
%used in the subsequent steps. The % major larger amount of computation
%occurs in the iterative computation step: % , and it can be divided into 4
%stages: (1) Compute the unstructured grid to identify the locations where
%analogs are computed; (2) Distribute the analog computation to the available
%computing resources; (3) Aggregate the analogs computed at different
%locations; and (4) valuate the predictions, and determine if termination
%condition is met. % \begin{enumerate} %   \item Compute the unstructured
%grid to identify the locations where %   analogs are computed; %   \item
%Distribute the analog computation to the available computing %   resources;
%%   \item Aggregate the analogs computed at different locations; %   \item
%Evaluate the predictions, and determine if termination condition is %   met;
%% \end{enumerate} The iteration stops when a termination condition is met,
%which is either the exhaustion of the computational resources available, or
%an overall prediction error below a specified threshold. Finally, a
%post-processing task interpolates the data at each location to generate the
%forecast solution.
%\jhanote{... till here.}

%\jhanote{proposed alternative}

Figure~\ref{fig:psu-use-case} shows the workflow of the \gls{AUA} algorithm.
The workflow can be divided into 4 steps: initialization; preprocessing;
iterative computation; and post-processing. The initialization step specifies
the search space and the test space, and sets up starting parameters for the
\gls{AnEn}. The preprocessing step generates preparatory data that will be
used in the subsequent steps. The larger amount of computation occurs in the
iterative computation step: (1) Compute the unstructured grid to represent
the locations where analogs need to be computed; (2) Distribute the analog
computation to the available computing resources; (3) Aggregate the analogs
computed at different locations; and (4) evaluate the predictions, and
determine if the termination condition is met. The termination condition
could be either the exhaustion of the computational resources available, or
an overall prediction error below a specified threshold. Finally, a
post-processing task interpolates the analogs at each location to generate
the forecast solution.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/use_case_anen_pst.pdf}
    \caption{Adaptive unstructured analog algorithm
    workflow.}\label{fig:psu-use-case}
\end{figure}

We use the unstructured grid methodology based on the Delaunay triangulation
method~\cite{triangulation} to drive the algorithm. The algorithm starts by
generating a number of random triangles to partition the domain. At each
iteration, one point is selected within each triangle, and it is assigned a
value equal to the average of the triangle's vertices.  This estimated value
is compared to the analysis (true) value.  If the error is above a threshold,
this point will be used as a new vertex in the next iteration.  
EnTK can dynamically dedicate resources as needed.


\begin{comment}
    \begin{itemize}
        \item Intro:
            \begin{itemize}
                \item Description: Brief introduction about the science of the use
                    case.
                \item Use case application computational requirements
                \item Middleware requirements
            \end{itemize}
        \item Why EnTK\@:
            \begin{itemize}
                \item At 10000 feet:
                    \begin{itemize}
                        \item Simplification
                        \item Automation
                        \item Scalability
                        \item Sophistication
                    \end{itemize}
                \item Use case requires multiples tasks and stages
                \item Use case requires multiple iterations of both stages and tasks.
                    Automation?
                \item We don’t know ahead of time:
                    \begin{itemize}
                        \item how many computations and therefore
                        \item How many cores
                    \end{itemize}
                \item Evaluation of partial results can be performed at runtime. Does
                    this produce asynchronous pipelines (to be defined/determined)?
                \item Experiments:
                    \begin{itemize}
                        \item Where to we run the experiments?
                            \begin{itemize}
                                \item At least one machine (XSEDE, SuperMIC) but best to have
                                    multiple machines (HPC) to minimize the overheads of queue
                                    time and, possibly, compare different resource’s overheads.
                            \end{itemize}
                        \item Benchmarking: EnTK enables both serial and concurrent
                            execution of tasks. This allows for experiments of scalability to
                            evaluate the tradeoff between walltime and number of nodes. These
                            could be experiments to perform for the paper.
                        \item Number of stations per task: What is the sweet spot between
                            EnTK overheads and the number of stations for file so that the
                            number of idle nodes is minimized.
                        \item How did EnTK enable the design of your application?
                            Comparing performance between before EnTK and with EnTK.
                        \item Fault tolerance and resilience:
                            \begin{itemize}
                                \item Capture rate of failure and whether/how we recover.
                                \item What kind of errors happens?
                                \item Where errors are generated: from the kernel or EnTK?
                                \item What type of failure specifically pertains to the use
                                    case?
                                \item Do we restart just a task or do we need to redo the
                                    whole stage?
                                \item Do we recover from a walltime failure enabling the
                                    execution only of the tasks that have not been yet executed?

                                    \begin{figure}[t]

                                        \centering
                                        \includegraphics[width=.6\columnwidth]{figures/UC_AnEn_Workflow.png}
                                        \caption{Pseudoplot PSU experiment.}\label{fig:psu-exp1}
                                    \end{figure}

                            \end{itemize}
                    \end{itemize}
                \item Why we don’t use an existing workflow system?
                    \begin{itemize}
                        \item What EnTK allows to do that other systems do not?
                            \begin{itemize}
                                \item Enables large number of workflows each representing a
                                    different science question EnTK lower the barrier of
                                    reimplementation.
                                \item Set of ensembles, not dependences. PSU use case has
                                    minimal dependencies requirements.
                            \end{itemize}
                        \item Enables to think of the workflow design without:
                            \begin{itemize}
                                \item Limiting the number of stations to the number of nodes
                                    (resource allocation)
                                \item Using a structured allocation grid because it usually
                                    makes computation easier (and coordination of distributed
                                    execution)
                            \end{itemize}
                    \end{itemize}
            \end{itemize}
        \item Description of the workflow
            \begin{itemize}
                \item See the use case (possibly with addressing comments)
            \end{itemize}
    \end{itemize}
\end{comment}


